Safe and Practical GPU Acceleration in TrustZone

We present a holistic design for GPU-accelerated computation in TrustZone TEE. Without pulling the complex GPU software stack into the TEE, we follow a simple approach: record the CPU/GPU interactions ahead of time, and replay the interactions in the TEE at run time. This paper addresses the approach's key missing piece -- the recording environment, which needs both strong security and access to diverse mobile GPUs. To this end, we present a novel architecture called CODY, in which a mobile device (which possesses the GPU hardware) and a trustworthy cloud service (which runs the GPU software) exercise the GPU hardware/software in a collaborative, distributed fashion. To overcome numerous network round trips and long delays, CODY contributes optimizations specific to mobile GPUs: register access deferral, speculation, and metastate-only synchronization. With these optimizations, recording a compute workload takes only tens of seconds, which is up to 95% less than a naive approach; replay incurs 25% lower delays compared to insecure, native execution.

==> tab-env.tex <==
% !TeX root = main.tex

\begin{table}[t!]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/env} 
	%	\vspace{-5pt}		% use as needed
	\caption{Experimental setup used in evaluation}
%		\sys{}'s test platform used in experiments}
	\label{tab:env}
	%	\vspace{-5pt}		% use as needed
\end{table}

==> tab-version.tex <==
% !TeX root = main.tex

\begin{table}[]
	\centering
	\includegraphics[width=0.42\textwidth{}]{./figs/version} 
	\vspace{-5pt}		% use as needed
	\caption{Different versions of \sys{}}
	\label{tab:version}
	\vspace{-15pt}		% use as needed
\end{table}

%\begin{table}[]
%	\centering
%	\includegraphics[width=0.4\textwidth{}]{./figs/net-env} 
%	\vspace{-5pt}		% use as needed
%	\caption{Netowrks setup for evaluation}
%	\label{tab:net-env}
%	\vspace{-5pt}		% use as needed
%\end{table}
